Preparing quantum many-body scar states on quantum computers

Quantum many-body scar states are highly excited eigenstates of many-body systems that exhibit atypical entanglement and correlation properties relative to typical eigenstates at the same energy density. Scar states also give rise to infinitely long-lived coherent dynamics when the system is prepared in a special initial state having finite overlap with them. Many models with exact scar states have been constructed, but the fate of scarred eigenstates and dynamics when these models are perturbed is difficult to study with classical computational techniques. In this work, we propose state preparation protocols that enable the use of quantum computers to study this question. We present protocols both for individual scar states in a particular model, as well as superpositions of them that give rise to coherent dynamics. For superpositions of scar states, we present both a system-size-linear depth unitary and a finite-depth nonunitary state preparation protocol, the latter of which uses measurement and postselection to reduce the circuit depth. For individual scarred eigenstates, we formulate an exact state preparation approach based on matrix product states that yields quasipolynomial-depth circuits, as well as a variational approach with a polynomial-depth ansatz circuit. We also provide proof of principle state-preparation demonstrations on superconducting quantum hardware.

==> MPS_to_Unitary_construction.tex <==
Standard algorithms exist in converting a matrix product state (MPS) with $N$ sites and bond dimension $\chi$ into $N$ unitaries of width $\ceil{\log_{2}{2\chi}}$~\cite{PhysRevLett.91.147902, PhysRevLett.95.110503}. The goal here is then to describe how to represent individual scarred eigenstates $\ket{\mathcal{S}_{k}}$ as an MPS. We can then convert the MPS construction into unitary circuits for quantum state preparation. 

We can express a matrix product state with open boundary conditions as 
\begin{equation}
    \sket{\psi} = \sum_{\vec{s}}\bra{L}M^{s_{1}}M^{s_{2}}\ldots M^{s_{N}}\ket{R}\ket{\vec{s}},
\end{equation}
where $M^{s_{i}}$ are $\chi\times\chi$ matrices, and $\bra{L}$ and $\ket{R}$ are respectively $\chi$-dimensional  row and column vectors describing open boundary conditions. One can view an MPS as a representation of a deterministic finite automata (DFA), where the matrices $M$ act as a transition matrix for  the DFA states ~\cite{PhysRevA.78.012356}. Since $M$ is a $\chi\times\chi$ matrix, this DFA will have $\chi$ states, and $M^{s_{i}}_{(jk)}$ will be nonzero if the character $s_{i}$ takes the state $j$ to the state $k$. The bra $\bra{L}$ tells us what DFA states we start in, and the ket $\ket{R}$ determines the allowed final DFA states. It is important to note that the states in the DFA are different entities from quantum states. 


DFAs are used to represent regular expressions, or string expressions using a finite set of characters. To see how we can use this language to represent quantum states, consider $\ket{S_{2}}$ for $N = 4$:
\begin{equation}\label{eq:mps}
    \ket{S_{2}} = \frac{1}{\sqrt{3}}\left(\ket{0101} + \ket{1001} + \ket{1010}\right)
\end{equation}
The set of computational states in the quantum states form a language $\{\ket{0101}, \ket{1001}, \ket{1010}\}$ from which a regular expression can be constructed where the characters in the regular expression are spin states $\{\ket{0}, \ket{1}\}$. For the states $\ket{S_{k}}$, the regular expression is 
\[ \sket{0}^{*}\left[\sket{1} \sket{0} \sket{0}^{*}\right]^{k-1}\sket{1}\sket{0}^{*}, \]
where $^{*}$ is a Kleene star $(a^{*} = I + a + aa + aaa + ...)$, and $\left[.\right]^{m}$ means to repeat the term inside the bracket $m$ times.

The DFA that represents the regular expression for $\ket{S_{k}}$ is shown in figure~\ref{fig:proj_dicke_dfa}. 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/mps_figs/S_DFA.png}
    \caption{A DFA representation of the $\sket{S_k}$ state.}
    \label{fig:proj_dicke_dfa}
\end{figure}
It consists of $2k$ DFA states $\{B_{0}, B_{j,+}, B_{j,-}, B_{k}\}_{j=1\ldots k-1}$. The DFA starts at $B_{0}$. The first computational state can either be $\ket{0}$ which transitions you back to $B_{0}$ or $\ket{1}$ which transitions you to $B_{1,-}$. We denote this by 
\begin{align*}
B_{0}(\ket{0}) &\to B_{0}\\
B_{0}(\ket{1}) &\to B_{1,-}
\end{align*}
For the intermediate states, we have
\begin{align*}
B_{j,-}(\ket{0}) &\to B_{j,+}\\
B_{j,+}(\ket{0}) &\to B_{j,+}\\
B_{j,+}(\ket{1}) &\to B_{j+1,-}
\end{align*}
Finally, the DFA terminates at the final state $B_{k}$, where
\begin{align*}
B_{k-1,+}(\ket{1}) &\to B_{k}\\
B_{k}(\ket{0}) &\to B_{k}
\end{align*}
All these transition rules can be summarized by a transition matrix $M$, where $M_{(i,j)}$ gives the character needed to take the DFA from state  $i$ to state $j$:
\begin{align*}
&M_{(B_{0},B_{0})}      &=\ket{0}, &M_{(B_{0},B_{1,-})}  &=\ket{1},\\
&M_{(B_{j,-},B_{j,+})}  &=\ket{0},\\
&M_{(B_{j,+},B_{j+1,-})}&=\ket{1}, &M_{(B_{j,+},B_{j,+})}&=\ket{0},\\
&M_{(B_{k-1,+},B_{k})}  &=\ket{1}, &M_{(B_{k},B_{k})}    &=\ket{0}.
\end{align*}
The full matrix is then
\[
  \NiceMatrixOptions{code-for-first-row=\scriptstyle,code-for-last-row=\scriptstyle}
      M=\begin{pNiceMatrix}[first-row,last-col=10]
          B_{0} & B_{1,-} & B_{1,+} & B_{2,-} & B_{2,+} & \cdots & B_{k-1,-} & B_{k-1,+} & B_{k}\\
          \sket{0} & \sket{1} & 0 & 0 & 0 & \cdots & 0 & 0 & 0 & B_{0} \\
          0 & 0 & \sket{0} & 0 & 0 & \cdots & 0 & 0 & 0 & B_{1,-} \\
          0 & 0 & \sket{0} & \sket{1} & 0 & \cdots & 0 & 0 & 0 & B_{1,+} \\
          0 & 0 & 0 & 0 & \sket{0} & \cdots & 0 & 0 & 0 & B_{2,-} \\
          0 & 0 & 0 & 0 & \sket{0} & \cdots & 0 & 0 & 0 & B_{2,+} \\
          \vdots & \vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots & \vdots \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & \sket{0} & 0 & B_{k-1,-} \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & \sket{0} & \sket{1} & B_{k-1,+} \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & 0 & \sket{0} & B_{k} \\
      \end{pNiceMatrix}
\]
To obtain the matrices from Eq.~\ref{eq:mps}, separate this transition matrix as $M = M^{\ket{0}} + M^{\ket{1}}$, where
\begin{align*}
    \NiceMatrixOptions{code-for-first-row=\scriptstyle,code-for-last-row=\scriptstyle}
        M^{\ket{0}} &=\begin{pNiceMatrix}
          1 & 0 & 0 & 0 & 0 & \cdots & 0 & 0 & 0  \\
          0 & 0 & 1 & 0 & 0 & \cdots & 0 & 0 & 0  \\
          0 & 0 & 1 & 0 & 0 & \cdots & 0 & 0 & 0  \\
          0 & 0 & 0 & 0 & 1 & \cdots & 0 & 0 & 0  \\
          0 & 0 & 0 & 0 & 1 & \cdots & 0 & 0 & 0  \\
          \vdots & \vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots  \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & 1 & 0  \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & 1 & 0  \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & 0 & 1  \\
    \end{pNiceMatrix}\\ 
%      &= \sket{B_0}\sbra{B_0} + \sum_{j=1}^{k-1}\left(\sket{B_{j,-}}\sbra{B_{j,+}} + \sket{B_{j,+}}\sbra{B_{j,+}}\right) + \sket{B_k}\sbra{B_k} \\
    \NiceMatrixOptions{code-for-first-row=\scriptstyle,code-for-last-row=\scriptstyle}
        M^{\ket{1}}& =\begin{pNiceMatrix}
          0 & 1 & 0 & 0 & 0 & \cdots & 0 & 0 & 0  \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & 0 & 0  \\
          0 & 0 & 0 & 1 & 0 & \cdots & 0 & 0 & 0  \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & 0 & 0  \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & 0 & 0  \\
          \vdots & \vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots  \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & 0 & 0  \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & 0 & 1  \\
          0 & 0 & 0 & 0 & 0 & \cdots & 0 & 0 & 0  \\
    \end{pNiceMatrix}\\
      %&= \sket{B_0}\sbra{B_{1,-}} + \sum_{j=1}^{k-2}\sket{B_{j,+}}\sbra{B_{j+1,-}} + \sket{B_{k-1,+}}\sbra{B_k}
\end{align*}
That is, $M^{\ket{0}}$ is obtained by applying $\bra{0}$ to every entry in $M$, and similarly for $M^{\ket{1}}$. These are $2k\times2k$ matrices, and so the overall bond dimension of the MPS will be $2k$. Also, since we start at state $B_{0}$ and end at state $B_{k}$, the boundary vectors become
\begin{align*}
      \bra{L} &= \begin{pNiceMatrix} 1 & 0 & \cdots & 0 \end{pNiceMatrix} \\
      \ket{R} &= \begin{pNiceMatrix} 0 & \cdots& 0 & 1 \end{pNiceMatrix}^{T}
\end{align*}

Orthogonalizing the overall MPS in one direction results in $N$ unitary matrices of size $\ceil{\log_{2}{4k}}$. Using Gray codes, each of these unitaries can be decomposed into $\mathcal{O}(k)$ toffolis, where the toffolis span over $\mathcal{O}(\log{k})$ qubits~\cite{https://doi.org/10.48550/arxiv.quant-ph/0504100}. Each of these toffilis then require $\mathcal{O}(\left(\log{k}\right)^{2})$ CNOT gates. Hence, the circuit depth representing this state is $\mathcal{O}\left(Nk\left(\log{k}\right)^{2}\right)$. Figure~\ref{fig:qcmps} depicts an example MPS-to-circuit of the $\ket{S_{k}}$ state, with $N=6$ and  $k=2$. 
Here, 
\begin{align*}
U_{1} &= \begin{pmatrix}
-\sqrt{\frac{2}{5}} & -\sqrt{\frac{3}{5}} \\
 -\sqrt{\frac{3}{5}}& \sqrt{\frac{2}{5}}
\end{pmatrix} \\
U_{2} & = \begin{pmatrix}
\sqrt{\frac{1}{2}} & \sqrt{\frac{1}{2}} \\
\sqrt{\frac{1}{2}}& -\sqrt{\frac{1}{2}}
\end{pmatrix}\\
U_{3} &= \begin{pmatrix}
-\sqrt{\frac{1}{4}} & \sqrt{\frac{3}{4}} \\
 \sqrt{\frac{3}{4}} & \sqrt{\frac{1}{4}}
\end{pmatrix}\\
U_{4} &= \begin{pmatrix}
\sqrt{\frac{2}{3}} &  \sqrt{\frac{1}{3}} \\
\sqrt{\frac{1}{3}} & -\sqrt{\frac{2}{3}}
\end{pmatrix}\\
U_{5} &= \begin{pmatrix}
-\sqrt{\frac{1}{3}} & \sqrt{\frac{2}{3}} \\
 \sqrt{\frac{2}{3}} & \sqrt{\frac{1}{3}}
\end{pmatrix}
\end{align*}

\begin{figure*}
\centering
\begin{gather*}
\Qcircuit @C=.5em @R=0.5em @!R {
\lstick{\ket{0}} & \qw          &\qw        &\qw        & \qw       &\qw       &\qw \\
\lstick{\ket{0}} & \qw          &\qw        &\qw        & \qw       &\qw       &\qw \\
\lstick{\ket{0}} & \qw          & \qw       &\qw        & \qw       &\qw       &\qw \\
\lstick{\ket{0}} & \gate{U_{1}} & \ctrlo{1} & \ctrlo{1} &\gate{X}   &\ctrlo{1} &\qw \\
\lstick{\ket{0}} & \gate{X}     & \targ     & \ctrlo{1} &\ctrlo{-1} &\ctrlo{1} &\qw \\
\lstick{\ket{0}} & \qw          & \qw       & \targ     & \ctrl{-1} &\targ     &\qw \\
}
\Qcircuit @C=.5em @R=0.5em @!R {
\qw & \qw          &\qw           &\qw        &\qw       &\qw          & \qw       &\qw\\
\qw & \qw          &\qw           &\qw        &\qw       &\qw          & \qw       &\qw\\
\qw & \qw          &\gate{U_{2}}  &\ctrlo{1}  &\ctrlo{1} &\gate{U_{3}} & \ctrlo{1} &\qw\\
\qw & \targ        &\ctrlo{-1}    &\targ      &\ctrl{1}  &\ctrl{-1}    & \ctrl{1}  &\qw\\
\qw & \ctrlo{-1}   &\ctrlo{-1}    &\ctrlo{-1} &\targ     &\ctrlo{-1}   & \targ     &\qw\\
\qw & \qw          &\qw           &\qw        &\qw       &\qw          & \qw       &\qw\\
}
\Qcircuit @C=.5em @R=0.5em @!R {
\qw &\qw        &\qw         &\qw        &\qw        &\qw          &\qw       & \qw       & \qw        &\qw        &\qw\\
\qw &\qw        &\gate{U_{4}}&\ctrlo{1}  &\ctrlo{1}  &\gate{U_{5}} &\ctrlo{1} & \ctrlo{1} & \gate{X}   &\ctrlo{1}  &\qw\\
\qw &\targ      &\ctrlo{-1}  &\targ      &\ctrl{1}   &\ctrl{-1}    &\ctrl{1}  & \targ     & \ctrlo{-1} &\targ      &\qw\\
\qw &\ctrlo{-1} &\ctrlo{-1}  &\ctrlo{-1} &\targ      &\ctrlo{-1}   &\targ     & \ctrl{-1} & \ctrl{-1}  &\ctrl{-1}  &\qw\\
\qw &\qw        &\qw         &\qw        &\qw        &\qw          &\qw       & \qw       & \qw        &\qw        &\qw\\
\qw &\qw        &\qw         &\qw        &\qw        &\qw          &\qw       & \qw       & \qw        &\qw        &\qw\\
}
\Qcircuit @C=.5em @R=0.5em @!R {
\qw &\qw        &\gate{-X_{}}  &\ctrlo{1} &\ctrlo{1}  & \gate{-H}      & \ctrlo{1} &\qw\\
\qw &\targ      &\ctrlo{-1}    &\targ     &\targ      & \targ \qwx{-1} &\targ      &\qw\\
\qw &\ctrl{-1}  &\ctrl{-1}     &\ctrl{-1} &\ctrlo{-1} & \ctrlo{-1}     &\ctrlo{-1} &\qw\\
\qw &\qw        &\qw           &\qw       &\qw        & \qw            & \qw       &\qw\\
\qw &\qw        &\qw           &\qw       &\qw        & \qw            & \qw       & \qw\\
\qw &\qw        &\qw           &\qw       &\qw        & \qw            & \qw       & \qw \\
}
\end{gather*}
\caption{Circuit Diagram for the $\ket{\mathcal S_{k}}$ state with $N = 6$ and $k = 2$ using the MPS representation.}

\label{fig:qcmps}
\end{figure*}

\begin{figure*}[t!]
\centering
\begin{gather*}
\Qcircuit @C=.5em @R=0.5em @!R {
\lstick{\ket{0}} & \qw          &\qw        &\qw        & \qw       &\qw       &\qw \\
\lstick{\ket{0}} & \qw          &\qw        &\qw        & \qw       &\qw       &\qw \\
\lstick{\ket{0}} & \qw          & \qw       &\qw        & \qw       &\qw       &\qw \\
\lstick{\ket{0}} & \gate{U_{1}} & \ctrlo{1} & \ctrlo{1} &\gate{X}   &\ctrlo{1} &\qw \\
\lstick{\ket{0}} & \gate{X}     & \targ     & \ctrlo{1} &\ctrlo{-1} &\ctrlo{1} &\qw \\
\lstick{\ket{0}} & \qw          & \qw       & \targ     & \ctrl{-1} &\targ     &\qw \\
}
\Qcircuit @C=.5em @R=0.5em @!R {
\qw & \qw          &\qw           &\qw        &\qw       &\qw          & \qw       &\qw\\
\qw & \qw          &\qw           &\qw        &\qw       &\qw          & \qw       &\qw\\
\qw & \qw          &\gate{U_{2}}  &\ctrlo{1}  &\ctrlo{1} &\gate{U_{3}} & \ctrlo{1} &\qw\\
\qw & \targ        &\ctrlo{-1}    &\targ      &\ctrl{1}  &\ctrl{-1}    & \ctrl{1}  &\qw\\
\qw & \ctrlo{-1}   &\ctrlo{-1}    &\ctrlo{-1} &\targ     &\ctrlo{-1}   & \targ     &\qw\\
\qw & \qw          &\qw           &\qw        &\qw       &\qw          & \qw       &\qw\\
}
\Qcircuit @C=.5em @R=0.5em @!R {
\qw &\qw        &\qw         &\qw        &\qw        &\qw          &\qw       & \qw       & \qw        &\qw        &\qw\\
\qw &\qw        &\gate{U_{4}}&\ctrlo{1}  &\ctrlo{1}  &\gate{U_{5}} &\ctrlo{1} & \ctrlo{1} & \gate{X}   &\ctrlo{1}  &\qw\\
\qw &\targ      &\ctrlo{-1}  &\targ      &\ctrl{1}   &\ctrl{-1}    &\ctrl{1}  & \targ     & \ctrlo{-1} &\targ      &\qw\\
\qw &\ctrlo{-1} &\ctrlo{-1}  &\ctrlo{-1} &\targ      &\ctrlo{-1}   &\targ     & \ctrl{-1} & \ctrl{-1}  &\ctrl{-1}  &\qw\\
\qw &\qw        &\qw         &\qw        &\qw        &\qw          &\qw       & \qw       & \qw        &\qw        &\qw\\
\qw &\qw        &\qw         &\qw        &\qw        &\qw          &\qw       & \qw       & \qw        &\qw        &\qw\\
}
\Qcircuit @C=.5em @R=0.5em @!R {
\qw &\qw        &\gate{-X_{\phantom 4}}  &\ctrlo{1} &\ctrlo{1}  & \gate{-H}      & \ctrlo{1} &\qw\\
\qw &\targ      &\ctrlo{-1}    &\targ     &\targ      & \targ \qwx{-1} &\targ      &\qw\\
\qw &\ctrl{-1}  &\ctrl{-1}     &\ctrl{-1} &\ctrlo{-1} & \ctrlo{-1}     &\ctrlo{-1} &\qw\\
\qw &\qw        &\qw           &\qw       &\qw        & \qw            & \qw       &\qw\\
\qw &\qw        &\qw           &\qw       &\qw        & \qw            & \qw       & \qw\\
\qw &\qw        &\qw           &\qw       &\qw        & \qw            & \qw       & \qw \\
}
\end{gather*}
\caption{Circuit diagram for the $\ket{\mathcal D^m_{k}}$ state with $m = 6$ and $k = 2$ obtained from the MPS representation. The unitaries $U_1,\dots,U_5$ are listed in Eq~\eqref{eq:Us}}
\label{fig:qcmps}
\end{figure*}

==> initial_preparation_circuit_general.tex <==
\section{General initial state preparation circuit}
% \andy{This is my derivation for a generalized preparation circuit.}
\label{app:general_angle}

The initial state to be prepared is given by
\be
\ket{\xi} = \frac{1}{Z} \prod_{j=0}^{N - 1}
\lf[
1 + (-1)^{j} \xi P^{0}_{j-1} \sigma^{+}_{j} P^{0}_{j+1}
\rt]
\ket{\Omega}.
\ee
Here,
$\xi$ is a non-negative real number,
$P^{0}_{j} = \ketbra{0}{0}$ is the projector to $\sket{0}$ on the $j$-th qubit,
$\sigma^{+}_{j} = \ketbra{1}{0}$ is the $j$-th qubit raising operator, 
$\sket{\Omega} = \sket{00 \cdots 0}$ is the all-zero qubit state and
$Z$ is the normalization factor.
For open-boundary conditions, we take $P^{0}_{N} = P^{0}_{-1} = 1$.
Without loss of generality, we take the convention that $j=0$ is the rightmost term in the above product, i.e., $\prod_{j=0}^{N-1} V_j \sket{\Omega} = V_{N-1} V_{N-2} \cdots V_{0} \sket{\Omega}$.
In this convention, the $j+1$-th qubit is always in its zero state when applying each term of the product, and hence $P^{0}_{j+1}$ can be omitted. This means that
\be
\ket{\xi} = \frac{1}{Z} \prod_{j=0}^{N - 1}
\lf(
1 +  P^{0}_{j-1} x_j \sigma^{+}_{j}
\rt)
\ket{\Omega},
\ee
where $x_j = (-1)^{j} \xi$.
To facilitate the derivation, we introduce the projector $P^{1}_{j} = \ketbra{1}{1}$ to the qubit state $\sket{1}$ to rewrite the equation as
\be
\ket{\xi} = \frac{1}{Z} \prod_{j=0}^{N - 1}
\lf[
P^{1}_{j-1} \lf(1 \rt) + P^{0}_{j-1} \lf( 1 + x_j  \sigma^{+}_{j} \rt)
\rt]
\ket{\Omega}.
\ee
The term inside the square bracket is in the form of a control-rotation except that $( 1 + x_j  \sigma^{+}_{j} )$ is not a unitary operator.

To make it a unitary operator, we first introduce a set of real constants $\phi_j$ where their values will be determined later in this appendix.
We can divide each term in the product by $\phi_j$ to give
\be
\ket{\xi} = \frac{1}{Z'} \prod_{j=0}^{N - 1}
\lf[
P^{1}_{j-1} \lf(\frac{1}{\phi_j} \rt) + P^{0}_{j-1} \frac{1}{\phi_j}  \lf(1 + x_j  \sigma^{+}_{j} \rt)
\rt]
\ket{\Omega},
\ee
where $Z' = Z / \prod_j \phi_j$.
We next recognize that the one state $\sket{1}$ is only generated by the $\sigma^{+}_{j}$ operator. Hence, the factor $1/\phi_j$ associated with $P^{1}_{j-1}$ can be moved to be associated with the $\sigma^{+}_{j - 1}$ in the previous product term. We can write
\be
\ket{\xi} = \frac{1}{Z'} \prod_{j=0}^{N - 1}
\lf[
P^{1}_{j-1} + P^{0}_{j-1} \frac{1}{\phi_j} \lf( 1 + \frac{x_j}{\phi_{j+1}}  \sigma^{+}_{j} \rt)
\rt]
\ket{\Omega},
\ee
where $\phi_{N} = 1$.
Since $\sigma^{+}_{j}$ only acts on $\sket{0}$ in this equation, we have $\sigma^{+}_{j} \sket{0} = i \sigma^{y}_{j} \sket{0}$ where $\sigma^{y} = -i \ketbra{0}{1} + i \ketbra{1}{0}$. This allows us to write
\be
\ket{\xi} = \frac{1}{Z'} \prod_{j=0}^{N - 1}
\lf[
P^{1}_{j-1} + P^{0}_{j-1} \frac{1}{\phi_j} \lf( 1 + i \frac{x_j}{\phi_{j+1}}  \sigma^{y}_{j} \rt)
\rt]
\ket{\Omega}.
\ee
If we pick
\be
\label{app_eq:phi_value}
\phi_j = \sqrt{1 + \lf| \frac{x_j}{\phi_{j+1}} \rt|^2} \text{\ \ and \ \ } \phi_N = 1,
\ee
the operator associated with $P^{0}_{j-1}$ is unitary such that
\be
\frac{1}{\phi_j} \lf( 1 + i \frac{x_j}{\phi_{j+1}}  \sigma^{y}_{j} \rt)
= \cos\frac{\theta_j}{2} + i \sin \frac{\theta_j}{2} \sigma^{y}_{j}
= \mathrm{R}_{Y, j} (\theta_j),
\ee
where $\mathrm{R}_{Y, j}$ is the Y-rotation gate on $j$-th qubit and the rotation angle $\theta_j$ is given by
\be
\label{app_eq:rotation_angle}
\theta_j = 2 \, \mathrm{arg}  \lf( 1 + i \frac{x_j}{\phi_{j+1}}  \rt),
\ee
where $\phi_{j}$ is given recursively by \cref{app_eq:phi_value}.

We can summarize our result as
\be
\ket{\xi} = \frac{1}{Z'} \prod_{j=0}^{N - 1}
\lf[
P^{1}_{j-1} + P^{0}_{j-1}\mathrm{R}_{Y, j} (\theta_j)
\rt]
\ket{\Omega}.
\ee
Note that since all terms are unitary, $\frac{1}{Z'}$ is just a global phase factor not relevant for the state preparation and hence can be dropped.
Introducing $\czerory{j-1}{j}{\theta_j}$ being the control Y-rotation gate of angle $\theta_j$ triggered by the zero state of the $(j-1)$-th qubit to rotate the target qubit $j$, we have the preparation circuit written as
\be
	\ket{\xi} = 
	\lf[\prod_{j=1}^{N - 1} \czerory{j-1}{j}{\theta_j} \rt]
	\mathrm{R}_{Y, 0} (\theta_0)
	\ket{\Omega},
\ee
where $\theta_j$ is given by \cref{app_eq:rotation_angle}.


==> recursive_construction.tex <==
\section{Recursive construction}

The state $\ket{\xi}$ is a superposition of quantum many-body scar states
\begin{align}
    \ket{\xi} = \sum^{L/2-1}_{n=0} c_n \ket{\mathcal S_n},
\end{align}
where
\begin{align}
\label{eq:Sn}
    \ket{\mathcal S_n} = \frac{1}{n!\sqrt{\mathcal N(N,n)}}(Q^\dagger)^n\ket{\Omega}.
\end{align}
and
\begin{align}
    Q^\dagger = \sum^{N-1}_{i=2} (-1)^i\, P^0_{i-1}\sigma^+_{i}P^0_{i+1}.
\end{align}
The normalization factor in Eq.~\eqref{eq:Sn} is
\begin{align}
    \mathcal N(N,n) = \binom{N-n-1}{n},
\end{align}
which counts the number of ways of distributing $n$ $1$s among $N-n$ $0$s such that there are never two or more consecutive $1$s and the edge qubits are always in the $\ket{0}$ state. We are looking for a circuit to prepare the states $\ket{\mathcal S_n}$.

To construct a circuit, it is useful to draw a connection between these states and the Dicke states. This is achieved by observing that
\begin{align}
    \ket{\mathcal S_n} = \mathcal C\, \ket 0\otimes\ket{\tilde D^{N-2}_{n}}\otimes\ket 0,
\end{align}
where $\mathcal C=\prod_{i \text{ odd}}Z_i$ and where
\begin{align}
    \ket{\tilde D^{N}_n} = \frac{1}{\sqrt{\binom{N-n+1}{n}}}\, \mathcal P_{\rm fib}\sum_{\substack{x\in \{0,1\}^{N} \\ \text{wt}(x)=n}}\ket{x}
\end{align}
is the projection of the Dicke state into the Fibonacci Hilbert space.
The quantity $\text{wt}(x)$ is the Hamming weight of the bitstring $x$, defined as the number of $1$s appearing in the string.
Like the standard Dicke states, the projected Dicke states have a recursive structure as a function of $N$:
\begin{align}
\label{eq:D Recursion}
\begin{split}
    \ket{\tilde D^{N}_n} &= \sqrt{\frac{n}{N-n+1}}\ket{\tilde D^{N-2}_{n-1}}\otimes \ket{01}\\
    &\indent + \sqrt{\frac{N-2n+1}{N-n+1}}\ket{\tilde D^{N-1}_n}\otimes \ket{0}.
\end{split}
\end{align}
We aim to use this recursion relation to find an inductive construction for the circuit.

The inductive construction proceeds by demanding that there exist a circuit, $\tilde U_{N-1,n}$, that can prepare both $\ket{\tilde D^{N-2}_{n-1}}$ and $\ket{\tilde D^{N-1}_n}$ starting from different initial states, i.e.,
\begin{align}
\label{eq:Utilde def}
    \tilde U_{N-1,n}
    \begin{cases}
    \ket{0}^{\otimes N-2n+1}\otimes\ket{10}^{\otimes n-1} = \ket{\tilde D^{N-2}_{n-1}}\otimes \ket 0\\
    \ket{0}^{\otimes N-2n-1}\otimes\ket{01}^{\otimes n} = \ket{\tilde D^{N-1}_{n}}
    \end{cases}
    .
\end{align}
We then posit the inductive form
\begin{align}
    \tilde U_{N,n} = \tilde U_{N-1,n}\, \tilde U^{SCS}_{N,n},
\end{align}
where
\begin{widetext}
\begin{align}
\label{eq:U-SCS}
    \tilde U^{SCS}_{N,n}\ket{0}^{\otimes N-2n}\otimes\ket{01}^{\otimes n}
    &=\sqrt{\frac{n}{N-n+1}} \ket{0}^{\otimes N-2n}\otimes\ket{01}^{\otimes n-1}\otimes \ket{01}
    + \sqrt{\frac{N-2n+1}{N-n+1}} \ket{0}^{\otimes N-2n}\otimes \ket{10}^{\otimes n-1}\otimes \ket{10} \\
    &=\sqrt{\frac{n}{N-n+1}} \ket{0}^{\otimes N-2n+1}\otimes\ket{10}^{\otimes n-1}\otimes \ket{1} 
    + \sqrt{\frac{N-2n+1}{N-n+1}} \ket{0}^{\otimes N-2n-1}\otimes \ket{01}^{\otimes n}\otimes \ket{0}.
\end{align}
With these definitions, we see that
\begin{align}
    \tilde U_{N,n}\ket{0}^{\otimes N-2n}\otimes\ket{01}^{\otimes n}
    &= \sqrt{\frac{n}{N-n+1}} \tilde U_{N-1,n}\ket{0}^{\otimes N-2n+1}\otimes\ket{10}^{\otimes n-1}\otimes \ket{1}
    + \sqrt{\frac{N-2n+1}{N-n+1}} \tilde U_{N-1,n}\ket{0}^{\otimes N-2n-1}\otimes \ket{01}^{\otimes n}\otimes \ket{0}\\
    &= \sqrt{\frac{n}{N-n+1}} \ket{\tilde D^{N-2}_{n-1}}\otimes \ket 0 \otimes \ket{1}
    + \sqrt{\frac{N-2n+1}{N-n+1}} \ket{\tilde D^{N-1}_{n}}\otimes \ket{0}\\
    &= \ket{\tilde D^{N}_{n}},
\end{align}
\end{widetext}
where we applied Eq.~\eqref{eq:Utilde def} in the second-to-last line and Eq.~\eqref{eq:D Recursion} in the last line.

Note that the action of $\tilde{U}^{SCS}_{N,n}$ on the given basis state in Eq.~\eqref{eq:U-SCS} can be implemented using a single layer of $n$ many $XY$ gates. In principle, we can continue the recursion process several times to reach
\begin{eqnarray}
    \tilde{U}_{N,n} &=& \tilde{U}_{N-1,n} \tilde{U}_{N,n}^{SCS} \nonumber \\
    &=& \tilde{U}_{N-2,n} \tilde{U}_{N-1,n}^{SCS} \tilde{U}_{N,n}^{SCS} \nonumber \\
    &=& \dots \nonumber \\
    &=& \tilde{U}_{N-k,n} \tilde{U}_{N-(k+1),n}^{SCS} \tilde{U}_{N-(k+2),n}^{SCS} \dots \tilde{U}_{N-1,n}^{SCS} \tilde{U}_{N,n}^{SCS} \nonumber\\
\end{eqnarray}
As long as the only action required (is it though? what about other basis states?) is that given by Eq.~\eqref{eq:U-SCS}, and as long as $N-k \geq 2n$, we can continue to implement the operations $\tilde{U}_{N-k,n}^{SCS}$ using $n$ many $XY gates$. However, it is unclear when to terminate the recursion process, and how to implement the final unitary $\tilde{U}_{N-k,n}$. Note that $n$ never decreases during the recursion process.
